The Dagstuhl Beginners Guide to Reproducibility for Experimental Networking Research

Reproducibility is one of the key characteristics of good science, but hard to achieve for experimental disciplines like Internet measurements and networked systems. This guide provides advice to researchers, particularly those new to the field, on designing experiments so that their work is more likely to be reproducible and to serve as a foundation for follow-on work by others.

==> sections/acm-terminology.tex <==
\section{ACM Terminology}\label{ACM-terminology}

%\todo{Both Juergen Schoenwaelder and Olivier Bonaventure, proposed to %include the ACM terminologies for repeatability, replicability, %reproducibility early in the draft}, see~\cite{ACM-Artifact}.

Before we elaborate principles and best practices for reproducibility, we clarify terminology that is often confused in this context. In particular, we refer to the definition in~\cite{ACM-Artifact} for the differences between repeatability, replicability and reproducibility.
\begin{description}
    \item[Repeatability] stands for a researcher who can obtain the same results for her own experiment under exactly the same conditions, i.e., she can reliably repeat her own experiment ('Same team, same experimental setup').
    \item[Replicabilit] stands for a different researcher who can obtain the same results for an experiment under exactly the same conditions and using exactly the same artifacts, i.e., another independent researcher can reliably repeat an experiment of someone else ('Different team, same experimental setup').
    \item[Reproducibility] stands for a different independent researcher who can obtain the same results for an experiment under different conditions and using her self-developed artifacts ('Different team, different experimental setup').
\end{description}

\begin{table}[t]
    \caption{ACM terminology on repeatability, replicability, and reproducibility~\cite{ACM-Artifact}.}
    \label{tab:my_label}
    \centering
    \begin{tabular}{lll}
      \toprule
        & \multicolumn{2}{c}{Level of change} \\ \cmidrule(r){2-3}
        Term  &  Team & Setup \\ \midrule
         \emph{Repeatability}  &  Same & Same \\
         \emph{Replicability}   &  Different & Same \\
         \emph{Reproducibility}   &  Different & Different \\
      \bottomrule
    \end{tabular}

\end{table}
